Axiomatic constraint systems for proof search modulo theories

Goal-directed proof search in first-order logic uses meta-variables to delay the choice of witnesses; substitutions for such variables are produced when closing proof-tree branches, using first-order unification or a theory-specific background reasoner. This paper investigates a generalisation of such mechanisms whereby theory-specific constraints are produced instead of substitutions. In order to design modular proof-search procedures over such mechanisms, we provide a sequent calculus with meta-variables, which manipulates such constraints abstractly. Proving soundness and completeness of the calculus leads to an axiomatisation that identifies the conditions under which abstract constraints can be generated and propagated in the same way unifiers usually are. We then extract from our abstract framework a component interface and a specification for concrete implementations of background reasoners.

==> Macros/Macros_10Fomega.tex <==
%Reduction rules
\newcommand\limp{\Rightarrow}

\newcommand{\andorl}{{\land\lor_l}}
\newcommand{\andorr}{{\land\lor_r}}
\newcommand{\andor}{\andorl,\andorr}
\newcommand{\ea}{\forall\exists}
\newcommand{\redF}{\FomegaC}

%Derivability

\newcommand\DerFomT[3]{\Deri[\FomegaC]{#1}{#2}{#3}}
\newcommand\DerFomTs[4]{\Deris[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\Derwf[2]{\textsf{wf}_{#1}(#2)}
\newcommand\DerFomt[4]{\Derif[\FomegaC]{#1}{#2}{#3}{#4}}
\newcommand\DerFomp[3]{\Derif[\FomegaC]{#1}{#2}{#3}\diamond}

%Syntax
%Kinds

\newcommand\Arr[2]{{#1}\rightarrow {#2}}

%Types
\newcommand{\varT}{\textsf{Var}^T}
\newcommand{\fall}[3][{}]{\forall{#2}^{#1}.{#3}}
\newcommand{\xists}[3][{}]{\exists{#2}^{#1}.{#3}}
\newcommand{\et}[2]{{#1}\wedge {#2}}
\newcommand{\ou}[2]{{#1}\vee {#2}}
%\newcommand{\impl}[2]{{#1}\arr {#2}}
\newcommand{\nega}[1]{\overline{#1}}
\newcommand{\non}[1]{{#1}^{\perp}}
\newcommand{\lamb}[3]{\lambda{#2}^{#1}.{#3}}
\newcommand{\dual}[1]{{#1}^{\bot}}
\newcommand{\bidual}[1]{{#1}^{\bot\bot}}
\newcommand{\tridual}[1]{{#1}^{\bot\bot\bot}}

\newcommand\xistscod[3][{}]{\exists^{\textsf{cod}}{#2}^{#1}.{#3}}
\newcommand{\etcod}[2]{{#1}\wedge^{\textsf{cod}} {#2}}
\newcommand{\oucod}[2]{{#1}\vee^{\textsf{cod}} {#2}}


%Terms
\newcommand\proji[2]{#1}
\newcommand\projii[2]{#2}

\newcommand{\var}{\textsf{Var}}

%\newcommand{\lamc}[4][{}{}]{{#2}^{\i #1}{#3}^{\ii #1}.{#4}}
%\newcommand\stac[2]{{#1}\cdot{{#2}}}
\newcommand{\inj}[4][{}{}]{\lambda #2^{\proji #1}#3^{\projii #1}.{#4}}
\newcommand\paire[2]{\langle{#1},{#2}\rangle}
%\newcommand{\switch}[1]{\bullet #1}

\newcommand{\Lamb}[3]{\Lambda{#2}^{#1}.{#3}}
\newcommand{\appl}[2]{\langle #1,#2\rangle}

\newcommand{\cutc}[2]{\{#1\sep#2\}}

\newcommand{\m}[3][{}]{\mu #2^{#1}\!.{#3}}
%\newcommand{\mt}[3][{}]{\tilde\mu {#2}^{#1}.{#3}}



%Semantics:

\newcommand{\semK}[1]{[\![#1]\!]}
\newcommand{\swapK}[2]{\textsf{swap}_{#1}{#2}}

\newcommand{\sem}[2]{[\![#2]\!]_{#1}}
\newcommand{\semt}[1]{[\![#1]\!]}

\newcommand{\orth}[2]{{#1\mathrel{{\perp}}#2}}

\newcommand{\effac}[1]{\|{#1}\|}
\newcommand{\twt}{\mathcal{T}}

\newcommand{\mU}{\mathcal U}
\newcommand{\mV}{\mathcal V}

\newcommand{\fp}[2]{\Phi_{#1}{#2}}
\newcommand\LamC[1]{\Lambda\_.{#1}}
\newcommand\applC[1]{\appl{\_}{#1}}

%======================
%Relationship with other formalisms

\newcommand\FFc[2][]{\delambda[#1]{(#2)}}
\newcommand\FFct[2]{\delambda({#2},{#1})}
\newcommand\FFctv[1]{\delambda{(#1)}}
\newcommand\FcFp[1]{{#1}^+}
\newcommand\FcFm[1]{{#1}^-}
\newcommand\FcFt[1]{#1^\dagger}
\newcommand\cstc{{\textsf{C}}}

\newcommand\FFctvname{\delambda[\textsf{V}]}

%Derivability in Fomega normal

\newcommand\DerFomiT[3]{\Deri[\Fomega]{#1}{#2}{#3}}
\newcommand\DerFomitwf[2]{\textsf{wf}^{#1}_{\Fomega}(#2)}
\newcommand\DerFomit[4]{\Derif[\Fomega]{#1}{#2}{#3}{#4}}

\newcommand\SNC{\SN{\B'\x'}_{\textsf{TC}}}
\newcommand\SNl{\SN{\B'\x'}_{\textsf{TL}}}


==> Macros/Macros_1Basics.tex <==
%Relations

\newcommand\red{\rightarrow}

\newcommand\inve[1]{{#1}^{-1}}
\newcommand\co[2]{{#1}\cdot{#2}}
\newcommand\Id[1][]{\textsf{Id}_{#1}}
\newcommand\suc[2]{\hspace{0.1cm}#1\hspace{-0.1cm}(#2)}
\newcommand\induced[2]{{#1}[#2]}

\newcommand\restr[2]{{#1}_{|#2}}

%Normalisation
\newcommand\patriarchal{patriarchal}
\newcommand\paternal{paternal}

\newcommand\rf[1]{\textsf{rf}^{#1}}
\newcommand\nf[1]{\textsf{nf}^{#1}}
\newcommand\SN[1]{\textsf{SN}^{#1}}
\newcommand\BN[2]{\textsf{BN}^{#1}_{#2}}
\newcommand\WN[1]{\textsf{WN}^{{#1}}}

\newcommand\RM[1]{\mathcal M_{#1}}
\newcommand\Remul{\mathcal W}
\newcommand{\multiset}[1]{\{ \!\! \{ #1\} \!\! \} }
\newcommand{\set}[1]{\{ #1\} }

\newcommand\lex{{\textsf{lex}}}
\newcommand\mul{{\textsf{mul}}}
\newcommand\lexx{{\textsf{lexx}}}
\newcommand\mull{{\textsf{mull}}}


%RPO=========================================

\newcommand{\llex}[1][<]{{#1}_{\lex}}
\newcommand{\glex}[1][>]{{#1}_{\lex}}

\newcommand{\lmul}[1][<]{{#1}_{\mul}}
\newcommand{\gmul}[1][>]{{#1}_{\mul}}

\newcommand{\lllex}[1][<]{{#1}_{\lexx}}
\newcommand{\gllex}[1][>]{{#1}_{\lexx}}

\newcommand{\lmull}[1][<]{{#1}_{\mull}}
\newcommand{\gmull}[1][>]{{#1}_{\mull}}

\newcommand\RPO{{\textsf{RPO}}}
\newcommand\LPO{{\textsf{LPO}}}
\newcommand\MPO{{\textsf{MPO}}}

\newcommand{\grpo}{\mbox{$>\!\!>$}}
\newcommand{\lrpo}{\mbox{$<\!\!<$}}

\newcommand{\glpo}{\mbox{$>\!\!>$}}
\newcommand{\llpo}{\mbox{$<\!\!<$}}

\newcommand{\gmpo}{\mbox{$>\!\!>$}}
\newcommand{\lmpo}{\mbox{$<\!\!<$}}

\ignore{
\newcommand{\grpo}[1][>]{{{#1}_{\textsf{rpo}}}}
\newcommand{\lrpo}[1][<]{{{#1}_{\textsf{rpo}}}}

\newcommand{\glpo}[1][>]{{{#1}_{\textsf{lpo}}}}
\newcommand{\llpo}[1][<]{{{#1}_{\textsf{lpo}}}}

\newcommand{\gmpo}[1][>]{{{#1}_{\textsf{mpo}}}}
\newcommand{\lmpo}[1][<]{{{#1}_{\textsf{mpo}}}}
}

\newcommand\pre{\prec}


%1st-order syntax======================================

\newcommand{\blob}{\star}
\newcommand\blobx[1]{\textsf{c}^{#1}}

\newcommand\uni[2]{\textsf{uni}(#1)}
\newcommand\bi[2]{\textsf{ii}(#1,#2)}

\newcommand\un[1]{\textsf{i}(#1)}
\newcommand\deux[2]{\textsf{ii}(#1,#2)}
\newcommand\two[2]{{\textsf{II}(#1,#2)}}

\newcommand\folet[2]{\textsf{let}(#1,#2)}
\newcommand\foap[2]{\textsf{ap}(#1,#2)}


\newcommand\varl[1]{\textsf{par}(#1)}
\newcommand\vart[2]{\textsf{cut}(#1,#2)}
\newcommand\coup[3][{}]{{\textsf{cut}}^{#1}(#2,#3)}
\newcommand\subf[3][{}]{\textsf{sub}^{#1}(#2,#3)}
\newcommand\subfc[2]{\textsf{subc}(#1,#2)}

\newcommand\focut[3][{}]{{\textsf{cut}^{#1}(#2,#3)}}
\newcommand\fosub[3][{}]{{\textsf{sub}^{#1}(#2,#3)}}

\newcommand\foP[3]{\deux {#2}{#3}}
\newcommand\folami[3]{\deux {#2}{#3}}
\newcommand\focontv[2]{\un{#2}}
\newcommand\focont[3][{}]{\focut[#1]{#2}{#3}}

\newcommand\foel{\blob}
\newcommand\foconc[2]{\deux {#1}{#2}}
\newcommand\fost[2]{\deux {#1}{#2}}

\newcommand\focuti[5][{}]{\fosub[#1]{#3}{#5}}


==> Macros/Macros_3CBV.tex <==
\newcommand\CPS{\textsf{CPS}}

%Moggi's lC
\newcommand\letinC[3]{\textsf{let }#2=#1\textsf{ in }{#3}}

\newcommand\bv{\beta_{\textsf V}}
\newcommand\ev{\eta_{\textsf V}}
\newcommand\evp{\eta'_{\textsf V}}


\newcommand\bl{{\textsf {B}}}
\newcommand\letC{{\textsf {let}}_{\textsf V}}
\newcommand\appleti{{\textsf {let}}_1}
\newcommand\appletii{{\textsf {let}}_2}
\newcommand\etalet{\eta_{\textsf {let}}}
\newcommand\letnesting{{\textsf {assoc}}}

%\newcommand\lCx{\lambda_{{\textsf C}\textsf{x}}}
\newcommand\lCb{\lambda_{{\textsf C}\beta}}
\newcommand\lCbe{\lambda_{{\textsf C}\beta\eta}}

%CPS-translations
\renewcommand\Re[1]{\mathcal{R}(#1)}
\newcommand\ReV[1]{\mathcal{R}_{\textsf V}(#1)}
\newcommand\Fi[1]{\mathcal{F}(#1)}
\newcommand\FiV[1]{\mathcal{F}_{\textsf V}(#1)}

\newcommand\Fis[2]{{#1}\colon_{\!\!\mathcal{F}}{#2}}
\newcommand\FisV[1]{{#1}^{\mathcal F}}
\newcommand\Rey[2]{{#1}\colon_{\!\!\mathcal{R}}{#2}}
\newcommand\ReyV[1]{{#1}^{\mathcal R}}

\newcommand\Fisback[1]{{#1}^{{\mathcal F}{\textsf {back}}}}
\newcommand\Fisbackname{{\mathcal F}{\textsf {back}}}


%Calculs CPS
\newcommand\lav{$\lambda_{\textsf {EvalArg}}$}
\newcommand\lContR{$\lambda^{\mathcal R}_{\CPS}$}
\newcommand\lContF{$\lambda^{\mathcal F}_{\CPS}$}
\newcommand\lContp{$\lambda_{\CPS}^+$}

\newcommand\lContRb{\lambda^{\mathcal R}_{\CPS\beta}}
\newcommand\lContRbe{\lambda^{\mathcal R}_{\CPS\beta\eta}}
\newcommand\lContFb{\lambda^{\mathcal F}_{\CPS\beta}}
\newcommand\lContFbe{\lambda^{\mathcal F}_{\CPS\beta\eta}}

\newcommand\lif[1]{\Uparrow{#1}}
\newcommand\lifname{\Uparrow}

%For later

\newcommand\lContfb{\lambda^{f}_{\CPS\beta}}
\newcommand\lContfbe{\lambda^{f}_{\CPS\beta\eta}}

\newcommand\nnot[1]{{#1}^{\bullet}}

\newcommand\liFf[1]{\uparrow{#1}}
\newcommand\liFfname{\uparrow}

\newcommand\cps[2]{{#1}\colon{#2}}
\newcommand\cpsV[1]{{#1}^{\dag}}

\newcommand\spc[1]{{#1}^{{\textsf {back}}}}
\newcommand\spcname{{(\_)}^{{\textsf {back}}}}

\newcommand\lContf{$\lambda^{f}_{\CPS}$}

\newcommand\lCont{\lambda_{\CPS}}

\newcommand\lConti{\lambda_{\textsf{cont}1}}
\newcommand\lContii{\lambda_{\textsf{cont2}}}

%To and from Moggi's C

\newcommand\Tii[1]{{#1}^{\sharp}}
\newcommand\Tiii[1]{{#1}^\natural}
\newcommand\Ti[1]{{#1}^\flat}

%\newcommand\Tiname{{(\_)}^\flat}
%\newcommand\Tiiname{{(\_)}^\sharp}
%\newcommand\Tiiiname{{(\_)}^\natural}


==> Macros/Macros_4LambdaI.tex <==
%lambda I

\renewcommand\corner[1]{\v{#1}}
\newcommand\wonalc{$\l^?$}
\newcommand\subanot[2]{#1\lhd{#2}}

\renewcommand\P[3]{\Pi {#1}^{#2}.{#3}}
\newcommand\lami[3]{\lambda {#1}^{#2}.{#3}}

\newcommand\dummy{\wp}
\renewcommand\i[1]{\textsf{i}({#1})}
\newcommand\iname{\textsf{i}}

\newcommand\typ{t}
\newcommand\betat{{\beta^{\typ}}}

\newcommand\pervar{\textsf{perp-var}}
\newcommand\perl{\textsf{perp}\lambda}
\newcommand\perlaa{\textsf{perp}\lambda^{\typ}_1}
\newcommand\perlab{\textsf{perp}\lambda^{\typ}_2}
\newcommand\perba{\textsf{perp}\beta_1}
\newcommand\perbb{\textsf{perp}\beta_2}
\newcommand\perbaa{\textsf{perp}\betat_1}
\newcommand\perbba{\textsf{perp}\betat_2}
\newcommand\perbca{\textsf{perp}\betat_3}
\newcommand\perpia{\textsf{perp}\Pi_1}
\newcommand\perpib{\textsf{perp}\Pi_2}

\newcommand\per{\rightsquigarrow}

\newcommand\RI[2]{{#1}\;\mathcal H\;{#2}}

\newcommand\GI[2]{{#1}\;\mathcal{G}\;{#2}}
\newcommand\Gax{\mathcal{G}\textsf{ax}}
\newcommand\Gvar{\mathcal{G}\textsf{var}}
\newcommand\Gl{\mathcal{G}\lambda}
\newcommand\Gla{\mathcal{G}\lambda^{\typ}}
\newcommand\Gba{\mathcal{G}\beta_1}
\newcommand\Gbb{\mathcal{G}\beta_2}
\newcommand\Gbaa{\mathcal{G}\betat_1}
\newcommand\Gbba{\mathcal{G}\betat_2}
\newcommand\Gweak{\mathcal{G}\textsf{weak}}
\newcommand\Gweaka{\mathcal{G}\textsf{weak1}}
\newcommand\Gweakb{\mathcal{G}\textsf{weak2}}
\newcommand\Gc{\mathcal{G}\textsf{c}}
\newcommand\Gpi{\mathcal{G}\textsf{$\Pi$}}

==> Macros/Macros_4SafeMin.tex <==
%PSN & Encodings to and from lambda=======================

\newcommand{\PSN}{{\textsf{PSN}}}


\renewcommand\H[1]{\textsf{H}({#1})}
\newcommand\Hname{\textsf{H}}
\newcommand\xtol[1]{\H{#1}}
\newcommand\xtolname{\Hname}

\newcommand\delambda[1][]{{\mathcal A}_{#1}}
\newcommand\alambda{{\mathcal B}}
\newcommand\dd[1]{\delambda(\alambda({#1}))}

\newcommand\kC[1]{{\delambda}_{\textsf{w}}{({#1})}}
\newcommand\kCCC[1]{{\delambda}{(#1)}}
\newcommand\kCC[2][]{{\delambda}_{#1}{(#2)}}
\newcommand\kCCname{{\delambda}}

\renewcommand\k[1]{\alambda{(#1)}}
\newcommand\kl[2]{\alambda^{#1}{(#2)}}
\newcommand\kname{{\mathcal B}}


%RPO encoding

\newcommand\polyx[1]{\overline{#1}}
\newcommand\polyxname{\overline {(\;)}}
\newcommand\polyxg[1]{\polyx{#1}}
\newcommand\polyxgname{\polyxname}


\newcommand\nb[1]{\sharp #1}

\newcommand\fo[1]{\polyx {#1}}
\newcommand\foe[1]{\polyx {#1}}
\newcommand\foename{\polyxname}

\newcommand\fot[1]{\polyx {#1}}
\newcommand\fotname{\polyxname}


\ignore{
\newcommand\polyx[1]{\mathcal P(#1)}
\newcommand\polyxname{\mathcal P}
}


%Safeness and minimality

\newcommand\safe[1]{\textsf{safe} {#1}}
\newcommand\minim[2]{\textsf{min}_{#1} #2}
\renewcommand\min[1]{\minim{}{#1}}

\newcommand{\unsafe}[1]{{\stackrel{\textsf{unsafe}}\longrightarrow}_{#1}\;}
\newcommand{\unsafen}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}
\newcommand{\unsafeplus}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{+}}_{#1}\;}
\newcommand{\undafesn}[1]{{{\stackrel{\textsf{unsafe}}\longrightarrow}^{*}}_{#1}\;}


%Lambda x
\newcommand\lamp[3]{\lambda {#1}.{#3}}
\newcommand\cuti[4]{\langle{#2}/{#3}\rangle{#4}}

\newcommand\x{\textsf{x}}



==> Macros/Macros_5Llxr.tex <==
\newcommand\strict{basic}
\newcommand\expsub{substitution constructor}

%Rewriting specific===========================

\newcommand{\Sim}[1]{\sim_{#1}\;}
\newcommand{\Rewmod}[2]{\rightarrow_{#1/#2}\;}
\newcommand{\Rewmodn}[2]{\rightarrow^{*}_{#1/#2}\;}

\newcommand{\LRewplus}[1]{\; \mbox{}_{#1}^{+}{\longleftarrow}\;}
\newcommand{\LRew}[1]{\; \mbox{}_{#1}{\longleftarrow}}
\newcommand{\LRewn}[1]{\; {\mbox{}_{#1\,}}^{*}{\longleftarrow}}
\newcommand{\RLRewn}[1]{{\longleftrightarrow}^{*}_{#1}}
\newcommand{\RLRew}[1]{{\longleftrightarrow}_{#1}}


\newcommand{\ssubst}[3]{\subst{#1}{#3}{#2}}
%\newcommand{\isubst}[2]{\{ #1 \backslash #2 \} }



%Terms===========================

\renewcommand\t{\textsf{r}}
\newcommand\xt{\textsf{xr}}
\newcommand{\weak}[2]{\mathcal{W}_{#1}(#2)}
\newcommand{\app}[4]{#1\; #3}

\newcommand{\clos}[2]{#2 {#1}}
\newcommand{\trip}[3]{\cuti{}{#2} {#1}}

%\newcommand{\clos}[2]{#1\langle #2\rangle}
%\newcommand{\trip}[3]{#1 =_{#3} #2}
%\newcommand{\iclos}[2]{#1[#2]}
\newcommand{\con}[4]{\mathcal{C}_{#1}^{#2\,|\,#3}(#4)}

\newcommand{\weakapp}[5]{\weak {#1}{\app {#2}{} {#4}{}}}

\newcommand{\wf}{\mbox{ \textsf{linear}}}

%Equations======================
\newcommand{\ac}{\textsf{A}_{\textsf{c}}}
\newcommand{\ccu}{\textsf{C}_{\textsf{c}}}
\newcommand{\ccd}{\textsf{P}_{\textsf{c}}}
\newcommand{\cw}{\textsf{P}_{\textsf{w}}}
\newcommand{\com}{\textsf{P}_{\textsf{s}}}
\newcommand{\cs}{\textsf{P}_\textsf{cs}}


%Rules============================

\newcommand\Abs{\textsf{Abs}}
\newcommand\Appi{\textsf{App1}}
\newcommand\Appii{\textsf{App2}}
\newcommand\Var{\textsf{Var}} 
\newcommand\Weaki{\textsf{Weak1}}
\newcommand\Weakii{\textsf{Weak2}}
\newcommand\Cont{\textsf{Cont}}
\newcommand\Comp{\textsf{Comp}}
\newcommand\WAbs{\textsf{WAbs}}
\newcommand\WAppi{\textsf{WApp1}}
\newcommand\WAppii{\textsf{WApp2}}
\newcommand\WSubs{\textsf{WSubs}} 
\newcommand\Merge{\textsf{Merge}}
\newcommand\Cross{\textsf{Cross}}
\newcommand\CAbs{\textsf{CAbs}}
\newcommand\CAppi{\textsf{CApp1}} 
\newcommand\CAppii{\textsf{CApp2}} 
\newcommand\CSubs{\textsf{CSubs}}

%Translation=================

\newcommand{\ord}[1]{{#1}}

%sn-x=========================
\newcommand\multip[2]{\mathcal M_{#1}({#2})}
\newcommand\Tcomplex[1]{\mathcal {T}\!\textsf{x} ({#1})}
\newcommand\pol[1]{\mathcal P({#1})}
\newcommand\polname{\mathcal P}

==> Macros/Macros_6G3.tex <==
%Strategies
\newcommand\princ{{\textsf{princ}}}
\newcommand\gauche{\textsf{left}}
\newcommand\droite{\textsf{right}}

\newcommand\simpl{{\textsf{s}}}
\newcommand\SI{{\textsf{SI}}}
\newcommand\KK{{\textsf{KK}}}
\newcommand\JC{{\textsf{JC}}}

\newcommand\CBV{\textsf{CBV}}
\newcommand\CBN{\textsf{CBN}}
\newcommand\CBVs{\textsf{CBV}_{\textsf{simple}}}
\newcommand\CBNs{\textsf{CBN}_{\textsf{simple}}}
\newcommand\CB{\textsf{CB}}
\newcommand\equCBV{\equiv_{\CBV}}
\newcommand\equCBN{\equiv_{\CBN}}

\newcommand\clas{\equiv}
\newcommand\mogo{\textsf{sc}}
\newcommand\quot{\textsf{nd}}

\newcommand\purq{\textsf{pur-q}}
\newcommand\purt{\textsf{pur-t}}
\newcommand\purGp{\textsf{pur}\Giiii'}
\newcommand\purGiv{\textsf{pur}\Giv}


%lambdabar

\newcommand\SVar{{\mathcal X}}
\newcommand\STerms{{\mathcal T}}
\newcommand\SLists{{\mathcal L}}

\newcommand\TSVar{{\mathcal Y}}
\newcommand\PSVar{{\mathcal X}}
\newcommand\TS{{\mathcal P}}
\newcommand\PSTerms{{\mathcal T}}
\newcommand\PSLists{{\mathcal L}}


\newcommand\cont[2]{{#1}\;{#2}}

\newcommand\el{[]}
\newcommand\conc[2]{{#1}@{#2}}
\newcommand\st[2]{{#1}\cdot{#2}}

%Typing
\newcommand\contr[1]{\textsf{select}_{#1}}

\newcommand\Air{\rightarrow\textsf{r}}
\newcommand\Ail{\rightarrow\textsf{l}}


%Term reduction rules
\newcommand\B{\textsf{B}}
\newcommand\Ai{\textsf{A1}}
\newcommand\Aii{\textsf{A2}}
\newcommand\Aiii{\textsf{A3}}
\newcommand\Bi{\textsf{B1}}
\newcommand\Bii{\textsf{B2}}
\newcommand\Biii{\textsf{B3}}
\newcommand\Ci{\textsf{C1}}
\newcommand\Cii{\textsf{C2}}
\newcommand\Ciii{\textsf{C3}}
\newcommand\Civ{\textsf{C4}}
\newcommand\Cv{\textsf{C5}}
\newcommand\Cvi{\textsf{C6}}
\newcommand\Cvii{\textsf{C7}}
\newcommand\Cviii{\textsf{C8}}
\newcommand\Di{\textsf{D1}}
\newcommand\Dii{\textsf{D2}}
\newcommand\Diii{\textsf{D3}}
\newcommand\Div{\textsf{D4}}
%\newcommand\Ei{\textsf{E}}
%\newcommand\Fi{\textsf{F}}

\newcommand\As{\textsf{As}}
\newcommand\Bs{\textsf{Bs}}
\newcommand\Cs{\textsf{Cs}}
\newcommand\CGs{\textsf{Cs}_{\textsf G}}
\newcommand\Ds{\textsf{Ds}}
\newcommand\Es{\textsf{E}}

==> Macros/Macros_7G4.tex <==
\def\ijcar{}
\def\journal{\ignore}
%=================================================

\newcommand{\Lveerto}{\mbox{$L\!\vee\!\rto$}}

\newcommand{\AB}{A\rto B}
\newcommand{\BA}{B\rto A}

\newcommand{\BC}{B\rto C}

\newcommand{\ABC}{(\AB) \rto C}
\newcommand{\CD}{C\rto D}
\newcommand{\DB}{D\rto B}
%\newcommand{\CB}{C\rto B}
\newcommand{\FG}{F\rto G}
\newcommand{\GH}{G\rto H}
\newcommand{\CDB}{(\CD)\rto B}
\newcommand{\FGH}{(\FG)\rto H}

\newcommand{\dec}[2]{\mbox{${#1}\!\colon\!{#2}$}}
\newcommand{\vA}{\mbox{$\dec{v}{A}$}}
\newcommand{\vB}{\mbox{$\dec{v}{B}$}}
\newcommand{\uC}{\mbox{$\dec{u}{C}$}}
\newcommand{\vC}{\mbox{$\dec{v}{C}$}}
\newcommand{\wA}{\mbox{$\dec{w}{A}$}}
\newcommand{\wB}{\mbox{$\dec{w}{B}$}}
\newcommand{\wC}{\mbox{$\dec{w}{C}$}}
\newcommand{\wD}{\mbox{$\dec{w}{D}$}}
\newcommand{\wE}{\mbox{$\dec{w}{E}$}}
\newcommand{\xA}{\mbox{$\dec{x}{A}$}}
\newcommand{\xB}{\mbox{$\dec{x}{B}$}}
\newcommand{\xC}{\mbox{$\dec{x}{C}$}}
\newcommand{\yA}{\mbox{$\dec{y}{A}$}}
\newcommand{\yB}{\mbox{$\dec{y}{B}$}}
\newcommand{\yC}{\mbox{$\dec{y}{C}$}}
\newcommand{\yD}{\mbox{$\dec{y}{D}$}}
\newcommand{\yE}{\mbox{$\dec{y}{E}$}}
\newcommand{\zA}{\mbox{$\dec{z}{A}$}}
\newcommand{\zB}{\mbox{$\dec{z}{B}$}}
\newcommand{\zC}{\mbox{$\dec{z}{C}$}}
\newcommand{\zD}{\mbox{$\dec{z}{D}$}}
\newcommand{\zE}{\mbox{$\dec{z}{E}$}}
\newcommand{\MA}{\mbox{$\dec{M}{A}$}}
\newcommand{\MB}{\mbox{$\dec{M}{B}$}}
\newcommand{\MD}{\mbox{$\dec{M}{D}$}}
\newcommand{\ME}{\mbox{$\dec{M}{E}$}}
\newcommand{\NA}{\mbox{$\dec{N}{A}$}}
\newcommand{\NB}{\mbox{$\dec{N}{B}$}}
\newcommand{\ND}{\mbox{$\dec{N}{D}$}}
\newcommand{\NE}{\mbox{$\dec{N}{E}$}}


                    
\ignore{
\newcommand{\esapp}[4]{\langle\!\langle #1/#2, #3,#4  \rangle    \!   \rangle}
\newcommand{\esappt}[3]{\langle\!\langle #1/#2, #3  \rangle    \!   \rangle}
\newcommand{\tesapp}[1]{\langle\!\langle #1 \rangle  \! \rangle}
\newcommand{\nomtesapp}{\langle\!\langle ~ \rangle \!\rangle}
\newcommand{\tsapp}[1]{\{\!\{ #1 \}  \! \}}
\newcommand{\nomtsapp}{\{ \! \{ ~ \} \! \}}
\newcommand{\sapp}[3]{\{\!\{#1/#2,#3 \}\! \}}
\newcommand{\ce}[2]{[\![#1/#2]\!]}
\newcommand{\nomcut}{cut}
\newcommand{\tcut}[2]{cut(#1,#2)}
\newcommand{\la}[4]{{\tt app}(#1,#2,#3.#4)}
\newcommand{\rew}{\rightarrow}
%\newcommand{\tra}[1]{{\cal T}(#1)}
\newcommand{\tra}[1]{\overline{#1}}
%\newcommand{\tce}[4]{[\![#4]\!]_{#1,#2,#3}}
\newcommand{\tce}[2]{[\![#2]\!]_{#1}}
\newcommand{\nomtce}{[\![~]\!]_{A}}
\newcommand{\tes}[2]{[#2]_{#1}}
\newcommand{\nomtes}{[~]_{A}}



\newcommand{\spred}{\triangleright}
\newcommand{\pair}[2]{\langle #1,#2\rangle}
\newcommand{\triple}[3]{\langle #1,#2,#3\rangle}
\newcommand{\app}[2]{app(#1,#2)}
\newcommand{\tapp}[3]{app(#2,#3)_{#1}}
\newcommand{\nomtapp}{app_{A}}
\newcommand{\msep}{\hspace{.5cm}}
}

\newcommand{\lam}[2]{\lambda {#1}.{#2}}
\newcommand{\leftz}[4]{#1[#2,#3.#4]}
\newcommand{\leftr}[6]{#1[#2.#3.#4,#5.#6]}
\newcommand{\inv}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninv}{{\tt inv}}
\newcommand{\inva}[2]{{\tt inva}(#1,#2)}
\newcommand{\invz}[3]{{\tt inv}(#1,#2.#3)}
\newcommand{\ninvz}{{\tt inv}}
\newcommand{\invr}[3]{{\tt inv}(#1,#2.#3)}

\newcommand{\type}[1]{\widehat{#1}}
%\newcommand{\of}[2]{#1 \; {\tt of }\; #2}
\newcommand{\of}[2]{{\tt of}(#1,#2)}
\newcommand{\nof}{{\tt of}}
\newcommand{\Of}{O\! f}
\newcommand{\Inv}{Inv}
\newcommand{\genax}[2]{{\tt Ax}(#1,#2)}
\newcommand{\decomp}[4]{{\tt dec}(#1,#2,#3.#4)}
\newcommand{\ndecomp}{{\tt dec}}
%\renewcommand{\ar}[3]{(#1 \rto #2) \rto #3}

\newcommand{\Cut}[3]{\letin {#1}{#2}{#3}}
\newcommand{\ncut}{{\tt cut}}

%========================
%Rewrite rules

\newcommand\decri{\textsf{d}1}
\newcommand\decrii{\textsf{d}2}
\newcommand\decriii{\textsf{d}3}
\newcommand\decriv{\textsf{d}4}
\newcommand\decrv{\textsf{d}5}
\newcommand\decrvi{\textsf{d}6}
\newcommand\decrvii{\textsf{d}7}
\newcommand\decrviii{\textsf{d}8}

\newcommand\cutri{\textsf{c}1}
\newcommand\cutrii{\textsf{c}2}
\newcommand\cutriii{\textsf{c}3}
\newcommand\cutriv{\textsf{c}4}
\newcommand\cutrv{\textsf{c}5}
\newcommand\cutrvi{\textsf{c}6}
\newcommand\cutrvii{\textsf{c}7}
\newcommand\cutrviii{\textsf{c}8}
\newcommand\cutrix{\textsf{c}9}

\ignore{
\newcommand\cutrx{\textsf{c}{10}}
\newcommand\cutrxi{\textsf{c}{11}}
\newcommand\cutrxii{\textsf{c}{12}}
\newcommand\cutrxiii{\textsf{c}{13}}
\newcommand\cutrxiv{\textsf{c}{14}}
\newcommand\cutrxv{\textsf{c}{15}}
\newcommand\cutrxvi{\textsf{c}{16}}
}

\ignore{
\newcommand\cutri{a}
\newcommand\cutrii{b}
\newcommand\cutriii{c}
\newcommand\cutriv{d}
\newcommand\cutrv{e}
\newcommand\cutrvi{f}
\newcommand\cutrvii{g}
\newcommand\cutrviii{\pi}
\newcommand\cutrix{\phi}
}
\newcommand\cutrx{\textsf{A}}
\newcommand\cutrxi{\textsf{B}}
\newcommand\cutrxii{\textsf{C}}
\newcommand\cutrxiii{\textsf{D}}
\newcommand\cutrxiv{\textsf{E}}
\newcommand\cutrxv{\textsf{F}}
\newcommand\cutrxvi{\textsf{G}}


\newcommand\invi{\textsf{i}1}
\newcommand\invii{\textsf{i}2}
\newcommand\inviii{\textsf{i}3}
\newcommand\inviv{\textsf{i}4}
\newcommand\invv{\textsf{i}5}
\newcommand\invvi{\textsf{i}6}
\newcommand\invvii{\textsf{i}7}
\newcommand\invviii{\textsf{i}8}

\newcommand\ofi{\textsf{o}1}
\newcommand\ofii{\textsf{o}2}
\newcommand\ofiii{\textsf{o}3}
\newcommand\ofiv{\textsf{o}4}

\newcommand{\lz}{L0 \rto}
\newcommand{\lrr}{L \rto\rto}

\ignore{
\newcommand{\lzn}{Lb}
\newcommand{\lrrn}{Li}
}
\newcommand{\lzn}{\textsf{I}}
\newcommand{\lrrn}{\textsf{K}}
\newcommand{\foA}{\textsf{I}}
%\newcommand{\fo}{\star}
\newcommand{\foI}{\textsf{J}}
\newcommand{\foO}{\textsf{J}}
\newcommand{\fodec}[1]{\textsf{D}^{#1}}
\newcommand{\foCut}[1]{\textsf{C}^{#1}}


\newcommand{\oid}{{\sf{ivdc}}}
\newcommand{\oidgs}{{\sf{ivdcgs}}}
\newcommand{\gs}{{\sf{gs}}}
\newcommand{\cegs}{{\sf{cegs}}}
\newcommand{\rs}{{\sf{rs}}}
\newcommand{\cers}{{\sf{cers}}}
\newcommand{\ars}{{\sf{ars}}}
\newcommand{\cears}{{\sf{cears}}}
\newcommand{\cbn}{{\sf{cbn}}}
\newcommand{\cecbn}{{\sf{cecbn}}}
\newcommand{\cbv}{{\sf{cbv}}}
\newcommand{\cecbv}{{\sf{cecbv}}}

\newcommand{\pr}{Principal}
\newcommand{\np}{Non-Principal}
\newcommand{\na}{Non-Auxiliary}
\newcommand{\au}{Auxiliary}

\def\kindi{\textsf{Kind}_1}
\def\kindii{\textsf{Kind}_2}
\def\kindiii{\textsf{Kind}_3}

%\def\myitem{\vspace{.5cm}\item}

\def\derivable#1{\infer{#1}{\ldots}}
\def\parag{}


==> Macros/Macros_8PTSC.tex <==
\newcommand\SCons{{\mathcal S}}

\newcommand\RSTerms{{\mathcal Z}}
\newcommand\K{\mbox{$\Box$}}
\newcommand\T{\star}
\newcommand\Rel{{\mathcal R}}
\newcommand\Sort{{\mathcal A}}

\newcommand\xsubst{\textsf{xsubst}}

%Typing======================================
\newcommand\emptyenv{[]}
\newcommand\conv{\Rewsn{\B\x}}


\newcommand\DPTSC{\vdash_{\PTSC}}

\renewcommand\wf[1][\PTSC]{\hspace{5 pt}\textsf{wf}_{#1}}
%Previous def in Part1/Llxr_Macros



\newcommand\empt{\textsf{empty}}
\newcommand\extend{\textsf{extend}}
\newcommand\Ttyped{\textsf{sorted}}
\newcommand\Picons{\Pi\textsf{wf}}
\newcommand\Pir{\Pi\textsf{r}}
\newcommand\Pil{\Pi\textsf{l}}
\newcommand\convr{\textsf{conv}_r}
\newcommand\convl{\textsf{conv}_l}

\newcommand\subenv{\sqsubseteq}

%PTS==================================
\newcommand\DPTS{\vdash_{\PTS}}
\newcommand\DeriCoC[3]{{#1}\DPTS {#2}\col{#3}}


==> Macros/Macros_9DB.tex <==
%Sequent calculus of constructions

\newcommand\PTSCdb{\PTSC_{\sf{db}}}
\newcommand\PTSCi{\PTSC_{\sf{imp}}}

\newcommand\STermsdb{{\mathcal T}_{\sf{db}}}
\newcommand\SListsdb{{\mathcal L}_{\sf{db}}}

\newcommand\Pdb[3]{\Pi^{#2}{#3}}
\newcommand\lamidb[3]{\lambda^{#2}{#3}}
\newcommand\liftdb[3]{U^{#1}_{#2}{(#3)}}

\newcommand\cutjdb[4]{{#4}\{\hspace{-3pt}\{{{#3}\!\leftarrow\!{#2}}\}\hspace{-3pt}\}}
\newcommand\eln{{[\!]}}
\newcommand\appli[2]{#1(#2)}

\newcommand\compsup[1]{\overline{\sf{im}}(#1)}

\newcommand\cogg[2]{\pi^{#1}{(#2)}}
\newcommand\coggg[2]{\rho^{#1}{(#2)}}
\newcommand\ccdb[2]{{#2},{#1}}
\newcommand\DBname[2]{\overline{#2}^{\,#1}}
\newcommand\nameDB[2]{\underline{#2}_{\,#1}}
\newcommand\cofinG[1]{\phi_{#1}}



%Term reduction rules
\newcommand\Bdb{\textsf{B}_{\sf{db}}}
\newcommand\Aidb{\textsf{A1}_{\sf{db}}}
\newcommand\Aiidb{\textsf{A2}_{\sf{db}}}
\newcommand\Aiiidb{\textsf{A3}_{\sf{db}}}
\newcommand\Bidb{\textsf{B1}_{\sf{db}}}
\newcommand\Biidb{\textsf{B2}_{\sf{db}}}
\newcommand\Biiidb{\textsf{B3}_{\sf{db}}}
\newcommand\Bivdb{\textsf{B4}_{\sf{db}}}
\newcommand\Cidb{\textsf{C1}_{\sf{db}}}
\newcommand\Ciidb{\textsf{C2}_{\sf{db}}}
\newcommand\Ciiidb{\textsf{C3}_{\sf{db}}}
\newcommand\Ciiiidb{\textsf{C3'}_{\sf{db}}}
\newcommand\Civdb{\textsf{C4}_{\sf{db}}}
\newcommand\Cvdb{\textsf{C5}_{\sf{db}}}
\newcommand\Cvidb{\textsf{C6}_{\sf{db}}}
\newcommand\Cviidb{\textsf{C7}_{\sf{db}}}
\newcommand\Cviiidb{\textsf{C8}_{\sf{db}}}
\newcommand\Didb{\textsf{D1}_{\sf{db}}}
\newcommand\Diidb{\textsf{D2}_{\sf{db}}}
\newcommand\Diiidb{\textsf{D3}_{\sf{db}}}
\newcommand\Divdb{\textsf{D4}_{\sf{db}}}

\newcommand\Asdb{\textsf{As}_{\sf{db}}}
\newcommand\Bsdb{\textsf{Bs}_{\sf{db}}}
\newcommand\Csdb{\textsf{Cs}_{\sf{db}}}
\newcommand\Dsdb{\textsf{Ds}_{\sf{db}}}

\newcommand\xdb{\textsf{x}_{\sf{db}}}

\newcommand\Alldb{\Bdb\xdb}


%Typing

\newcommand\DeriTIdbf[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIdbsf[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTIdb[3]{\Deri[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriTIdbs[4]{\Deris[{\sf{TS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTIdb{\hspace{5 pt}\textsf{wf}_{\sf{TS}_{\sf{db}}}}

\newcommand\TIdb{{\sf{TS}}_{\sf{db}}}
\newcommand\PSdb{{\sf{PS}}_{\sf{db}}}

\newcommand\DeriPSdb[3]{\Deri[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}}
\newcommand\DeriPSdbs[4]{\Deris[{\sf{PS}}_{\sf{db}}]{#1}{#2}{#3}{#4}}


==> Macros/Macros_9Enumeration.tex <==
\ignore{
\newcommand\enum[5]{#2\sep #3\Longrightarrow #4\sep #5}
\newcommand\enums[6]{#2;#3\sep #4\Longrightarrow #5\sep #6}
}

\newcommand\enum[5]{\Deri{#2}{#4}{#3}\sep {#5}}
\newcommand\enums[6]{\Deris{#2}{#3}{#5}{#4}\sep {#6}}
\newcommand\goals[2]{#1\Longrightarrow #2}

\newcommand\PE{\textsf{PE}}

\newcommand\enumPS[5]{\Derip{\PE}{#2}{#4}{#3}\sep {#5}}
\newcommand\enumPSs[6]{\Derip{\PE}{#2;#3}{#5}{#4}\sep {#6}}
\newcommand\goalsPS[2]{#1\Longrightarrow_{\PE} #2}


\newcommand\constr[3]{#2\stackrel{#1}\longleftrightarrow #3}


==> Macros/Macros_9ProofSearch.tex <==
%Proof search


\newcommand\DPS{\vdash_{\textsf{PS}}}
\newcommand\PSS{\textsf{PS}}


\newcommand\DeriPS[3]{{#1}\DPS {#2}\col{#3}}
\newcommand\DeriPSs[4]{{#1};{#2}\DPS {#3}\col{#4}}

\newcommand\TtypedPS{\textsf{sorted}_\textsf{PS}}
\newcommand\contrs[1]{\textsf{sel.}_{#1}}
\newcommand\axPS{\textsf{ax}_\textsf{PS}}
\newcommand\PiconsPS{\Pi\textsf{wf}_\textsf{PS}}
\newcommand\PirPS{\Pi\textsf{r}_\textsf{PS}}
\newcommand\PilPS{\Pi\textsf{l}_\textsf{PS}}



==> Macros/Macros_9Tsynth.tex <==
%TI

\newcommand\Deric[3]{\Deri{#1}{#2}{\equiv\! #3}}
\newcommand\Derics[4]{\Deris{#1}{#2}{#3}{\equiv\! #4}}



\newcommand\DeriTIf[3]{\Deri[{\textsf{TS}}]{#1}{#2}{\equiv\! #3}}
\newcommand\DeriTIsf[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{\equiv\! #4}}
\newcommand\DeriTI[3]{\Deri[{\textsf{TS}}]{#1}{#2}{#3}}
\newcommand\DeriTIs[4]{\Deris[{\textsf{TS}}]{#1}{#2}{#3}{#4}}
\newcommand\wfTI{\hspace{5 pt}\textsf{wf}_{\textsf{TS}}}

\newcommand\extendTI{\textsf{extend}_\textsf{TS}}
\newcommand\axTI{\textsf{ax}_\textsf{TS}}
\newcommand\PiconsTI{\Pi\textsf{wf}_\textsf{TS}}
\newcommand\PirTI{\Pi\textsf{r}_\textsf{TS}}
\newcommand\PilTI{\Pi\textsf{l}_\textsf{TS}}

\newcommand\convp{\Rewsn{\B\x}}

\newcommand\expimp[1]{\Downarrow\!(#1)}
\newcommand\expimpname{\Downarrow}
\newcommand\TI{\textsf{TS}}

==> Macros/Macros_Main.tex <==
%Miscellaneous========================
%\tracingall

\long\def\ignore#1{\relax}

\newcommand\figurefont{\fontsize{9}{11}}

\newcommand\struto[1][15pt]{{\raise #1 \hbox{\strut}}}%
\newcommand\strutb[1][15pt]{{\raise-#1 \hbox{\strut}}}%

\newcommand\upline{\hline\struto[5pt]}
\newcommand\midline[1][5pt]{\\[#1]\hline\struto[5pt]}
\newcommand\mmidline[1][5pt]{\\[#1]\hline\hline\struto[5pt]}
\newcommand\downline[1][5pt]{\\[#1]\hline}

%=================================================
%Floating figures WHERE I WANT====================

\renewcommand{\topfraction}{0.95}  % max fraction of floats at top
\renewcommand{\bottomfraction}{0.95}       % max fraction of floats at bottom
\renewcommand\floatpagefraction{.5}
\renewcommand\textfraction{0.1}   
\setcounter{totalnumber}{50}
\setcounter{topnumber}{50}
\setcounter{bottomnumber}{50}
 \floatsep5pt  
 \intextsep5pt 
%\abovecaptionskip1pt
%\belowcaptionskip2pt

% \makeatletter
% \def\@boxfigurewith[#1]{\figure[#1]\vbox\bgroup\hrule height.1em}
% \def\@boxfigurewithout{\figure\vbox\bgroup\hrule height.1em}
% \newenvironment{bfigure}{\@ifnextchar[\@boxfigurewith\@boxfigurewithout}{\vskip.2em\hrule height.1em\egroup\endfigure}
% \makeatother

%Footnote
\interfootnotelinepenalty=1000000000


%=======================================================
% New theorem environment, often missing from cls files

\newtheorem{warning}{Notice}


%=======================================================
% To write stuff in aux file

 \newcommand\toaux[1]{\immediate\write\@auxout{#1}}


%========================================================
% Renewing itemize environment (too much space otherwise)

\newcommand\flush{\vrule width0pt height0pt\hfill}

% \newcommand\olditem{}
% \newcommand\olditemize{}
% \newcommand\oldenditemize{}
% \newcommand\oldenumerate{}
% \newcommand\oldendenumerate{}
% \let\olditem\item
% \let\olditemize\itemize
% \let\oldenditemize\enditemize
% \let\oldenumerate\enumerate
% \let\oldendenumerate\endenumerate
% 
% 
% \newbox\itemlabbox
% \newdimen\itemlabwd
% \newdimen\itemizespacing
% \setlength\itemizespacing{0.2\baselineskip}%
% 
% \newcommand\myitem{}
% \makeatletter
% \def\myitem{%
% \@ifnextchar[\@myitemwith\@myitemwithout}
% \long\def\@myitemwith[#1]{\hrule height0pt%
%   \olditem[]%
%   \removelastskip\vskip\itemizespacing%
%   \leavevmode%
%   \hskip-\leftmargin
%   \setbox\itemlabbox=\hbox\bgroup\hfil#1\hfil\egroup%
%   \ifdim\wd\itemlabbox>\itemlabwd%
%   \box\itemlabbox%
%   \else\hbox to\itemlabwd{#1\hfill}\fi%
%   \rule[0pt]{0pt}{0pt}}
% \long\def\@myitemwithout{\removelastskip\hrule height0pt\olditem\unskip\vskip\itemizespacing\rule[0pt]{0pt}{0pt}}
% \makeatother
% 
% 
% \renewenvironment{itemize}[1][]{%
%   \removelastskip%
%   \setbox\itemlabbox=\hbox\bgroup\hfil#1\hfil\egroup%
%   \setlength\itemlabwd{\wd\itemlabbox}%
%   \def\item{\myitem}%
%   \widowpenalty=3000%
%   \nobreak%
%   \advance\leftmargini-10pt%
%   \advance\leftmarginii-5pt%
%   \olditemize%
%   \unskip%
%   \bgroup%
%   \setlength\parskip{\itemizespacing}%
%   \setlength\topsep{0pt}%
%   \setlength\partopsep{0pt}%
%   \setlength\parsep{0pt}%
%   \setlength\itemsep{0pt}%
%   \setlength\itemindent\parindent%
%   \setlength\listparindent\parindent%
% }
% {\removelastskip\hrule height0pt\nobreak\egroup\oldenditemize\unskip\vskip\itemizespacing%
%   \def\item{\olditem}%
% }
% 
% \renewenvironment{enumerate}[1][0]{%
%   \removelastskip%
%   \setbox\itemlabbox=\hbox\bgroup\hfil#1\hfil\egroup%
%   \setlength\itemlabwd{\wd\itemlabbox}%
%   \def\item{\myitem}%
%   \widowpenalty=3000%
%   \nobreak%
%   \advance\leftmargini-10pt%
%   \advance\leftmarginii-5pt%
%   \oldenumerate%
%   \unskip%
%   \bgroup%
%   \setlength\parskip{\itemizespacing}%
%   \setlength\topsep{0pt}%
%   \setlength\partopsep{0pt}%
%   \setlength\parsep{0pt}%
%   \setlength\itemsep{0pt}%
%   \setlength\itemindent\parindent%
%   \setlength\listparindent\parindent%
% }
% {\removelastskip\hrule height0pt\nobreak\egroup\oldendenumerate\unskip\vskip\itemizespacing%
%   \def\item{\olditem}%
% }


\newcommand\mybox[1]{\fbox{\vbox{#1}}}
%\newcommand\mycbox[1]{\fbox{\vbox{#1}}}
\newcommand\mycbox[1]{\begin{tabular}{|l|}\upline #1 \downline\end{tabular}}
%\newcommand\mycbox[1]{\fbox{\bgroup#1\egroup}}


%======================================================
% Renewing maths environment (too much space otherwise)

% \newcommand\oldparforMain{}
% \let\oldparforMain\par
% \newcommand\topequationskip{.2\baselineskip}
% \newcommand\botequationskip{.2\baselineskip}
% 
% \makeatletter
% \renewcommand\[[1][\topequationskip]{\begingroup\let\mysavedpar\par\let\par\oldparforMain\vskip#1\nopagebreak\hbox to\hsize\bgroup\hfil\(}
% \renewcommand\][1][\botequationskip]{\)\hfil\egroup\hrule height 0pt\endgroup%\@afterindentfalse\@afterheading
%   \vskip#1}
% \makeatother

%======================================================
% Macros to create columns

\newbox\columnsbox
\newbox\tmpbox
\newdimen\columnsheight
\newdimen\columnwidth
\newdimen\remainingwidth
\newdimen\textwidthsave
\def\mycolumnsheight{}

\newcommand\columns[1]{%
  \def\mycolumnsheight{}%
  \setlength\remainingwidth\textwidth%
  \setbox\columnsbox=\vbox\bgroup\vskip0pt\vfil\hbox to\textwidth\bgroup#1\egroup\vfil\egroup%
  \columnsheight=\ht\columnsbox%
  \def\mycolumnsheight{to\columnsheight}%
  \hrule height 0pt\vtop{\hbox to\wd\columnsbox\bgroup#1\egroup}%
}

\makeatletter

\def\commonpart{%
  \setlength\columnwidth{\wd\tmpbox}%
  \vtop{\vskip0pt\hbox to\columnwidth{{\box\tmpbox}}}%
  \advance\remainingwidth-\columnwidth%
  \setlength\textwidth\textwidthsave%
  \hsize\textwidthsave%
}
\def\column{\unskip\setlength\textwidthsave\textwidth\@ifnextchar[\@columnwith\@columnwithout}
\long\def\@columnwith[#1]#2{%
  \def\newhsize{#1\dimexpr\textwidth\relax}%
  \hsize\newhsize%
  \ifdim\hsize<0.1pt\hsize\remainingwidth\fi%
  \setlength\textwidth\hsize%
  \setbox\tmpbox=\hbox to\hsize\bgroup\hfil\vtop\mycolumnsheight{\vskip0pt#2\vskip0pt}\hfil\egroup%
  \commonpart%
}
\long\def\@columnwithout#1{%
  \hsize\remainingwidth%
  \setlength\textwidth\hsize%
  \setbox\tmpbox=\hbox\bgroup\vtop\mycolumnsheight{\vskip0pt#1\vskip0pt}\egroup%
  \commonpart%
}
\makeatother

\newcommand\cquad[1][.01]{\column[#1]{}}

\newcommand\xtextwidth[1]{#1\dimexpr\hsize\relax}
\newcommand\xtextheight[1]{#1\dimexpr\vsize\relax}

\newenvironment{centre}{\begin{center}\unskip}{\end{center}\unskip}
\newcommand\ctr[1]{\begin{centre}#1\end{centre}}


%General====================================================
\newcommand\abs[1]{{\left|#1\right|}}        % val.absolue
\newcommand\mn[1]{{\overline{#1}}}                   % moyenne
\newcommand\vect[1]{{\overrightarrow{#1}}}            % vecteur
\newcommand\M[1]{{\mathcal{#1}}}                     % grandeurs molaires
\newcommand\ti[1]{\widetilde{#1}}
\newcommand\unif{\bigcap}
\newcommand\unit{\textsf{unit}}
\newcommand\sub{\subseteq}
\newcommand\N{\mathbb{N}}
\newcommand\corner[1]{\langle #1 \rangle}

%Abbrev==================================================

\newcommand\ith{${}^{\text{th}}$}
\renewcommand{\iff}{if and only if}
\newcommand{\mand}{\mbox{ and }}
\newcommand{\ie}{i.e.~}
\newcommand{\eg}{e.g.~}
\newcommand{\cf}{cf.~}
\newcommand{\etc}{etc.~}
\newcommand{\wrt}{w.r.t.~}
\newcommand{\resp}{resp.~}
\newcommand{\aka}{a.k.a~}
\newcommand{\ih}{\mbox{by i.h.}}

%Maths======================================================
\newcommand\dom[1]{\textsf{Dom}{(#1)}}
\newcommand\card[1]{|#1|}
\newcommand\maxi{\textsf{max}}
\newcommand{\sm}{\setminus}
\newcommand{\es}{\emptyset}
\newcommand{\eqdef}{:=\ }
\newcommand{\recdef}{::=\ }
\newcommand{\sqin}{\textsf{\footnotesize{E}}}
\newcommand{\sqes}{\not{\mbox{\![\hspace{-0.02cm}]}}}
\newcommand*{\longhookrightarrow}{\ensuremath{\lhook\joinrel\relbar\joinrel\relbar\joinrel\rightarrow}}
\newcommand\powerset[1]{\mathds P(#1)}

%Greek======================================================
\renewcommand\a{\alpha}
\renewcommand\b{\beta}
\newcommand\g{\gamma}
\renewcommand\d{\delta}
\renewcommand\l{\lambda}
%\newcommand\m{\mu}
\newcommand\clambda{\mbox{$\lambda\hspace{-5.4pt}\lambda$}}


\newcommand{\Gam}{\Gamma}
\newcommand{\Gm}{\mbox{$\Gamma$}}
\newcommand{\Lam}{\Lambda}
\newcommand{\Del}{\Delta}
\newcommand{\Ups}{\Upsilon}
\newcommand{\Om}{\Omega}
\newcommand{\Sig}{\Sigma}
\newcommand{\sig}{\sigma}
\newcommand{\cals}{{\mathcal S}}
\newcommand{\calf}{{\mathcal F}}

\newcommand\gGamma{\mathfrak{G}}
\newcommand\gDelta{\mathfrak{H}}
\newcommand\gA{\mathfrak{A}}
\newcommand\gB{\mathfrak{B}}
\newcommand\gC{\mathfrak{C}}
\newcommand\gP{\mathfrak{P}}



%Logical systems & Calculi==================================

\newcommand\NJ{\textsf{NJ}}
\newcommand\LJ{\textsf{LJ}}
\newcommand\LK{\textsf{LK}}
%\newcommand\LKmm{$\textsf{LK}_{\mu\tilde\mu}$}

\newcommand\Gzs{\textsf{G1}}
\newcommand\Gz{\textsf{G1ii}}
\newcommand\Giiis{\textsf{G3}}
\newcommand\Giii{\textsf{G3ii}}
\newcommand\Giiii{\Giii}
\newcommand\Gthree{\Giii}

\newcommand\LJT{\textsf{LJT}}
\newcommand\LJQ{\textsf{LJQ}}
\newcommand\LJF{\textsf{LJF}}
\newcommand\LKT{\textsf{LKT}}
\newcommand\LKQ{\textsf{LKQ}}
\newcommand\LKF{\textsf{LKF}}
\newcommand\LAF[1][]{$\textsf{LAF}_{#1}$}
\newcommand\LAFcf[1][]{$\textsf{LAF}^{\textsf{cf}}_{#1}$}

\newcommand{\LJQp}{\ensuremath{\mathbf \LJQ^\prime}}

\newcommand\Giv{\textsf{G4ii}}
\newcommand\Gfour{\Giv}

\newcommand\lG{\l\textsf{G3}}
\newcommand\lGcf{\l\textsf{G3}^{\textsf{cf}}}
\renewcommand\S{\textsf{S}}

\newcommand\lb{$\overline{\lambda}$}
\newcommand\lbm{\overline{\lambda}}
\newcommand\lLJQ{$\l\LJQ$}
\newcommand\lLJQm{\l\LJQ}

\newcommand\lk{$\lambda\xi$}
\newcommand\lm{$\lambda\mu$}
\newcommand\Lm{$\overline{\lambda}\mu$}
\newcommand\Lmm{$\overline{\lambda}\mu\widetilde{\mu}$}

\newcommand\LI{$\lambda I$}
\newcommand\Li{\Lambda I}

\newcommand\lx{$\l${\textsf x}}

\newcommand\lxx{$\l${\textsf {xx}}}

\renewcommand\ll{\lambda \textsf{lxr}}
\newcommand\lle{\l{\textsf {lxr}}}
\newcommand\Ll{$\lambda$l\textsf{xr}}

\newcommand\lC{$\l_{\textsf C}$}
\newcommand\lV{$\l_{\textsf{V}}$}

\newcommand\mathFomega{F_\omega}
\newcommand\Fomega{\ifmmode\mathFomega\else$\mathFomega$\fi}
\newcommand\mathFomegaC{F_\omega^{\mathcal C}}
\newcommand\FomegaC{\ifmmode\mathFomegaC\else$\mathFomegaC$\fi}
\newcommand\mathDNE{\mathrm{DNE}}
\newcommand\DNE{\ifmmode\mathDNE\else$\mathDNE$\fi}

\newcommand\PTS{{\textsf{PTS}}}
\newcommand\PTSC{{\textsf{PTSC}}}

\newcommand\CoC{{\textsf{CoC}}}
\newcommand\Coq{{\textsf{Coq}}}
\newcommand\coqide{\texttt{coqide}}
\newcommand\Lego{{\textsf{Lego}}}
\newcommand\CoS{{\textsf{CoS}}}

\newcommand\KSf{\textsf{KSf}}
\newcommand\SKSf{\textsf{SKSf}}

\newcommand\KSfl{{\textsf {KSfl}}}
\newcommand\SKSfl{{\textsf {SKSfl}}}

% \newcommand\FA{{Formalism \textsf {A}}}
% \newcommand\FB{{Formalism \textsf {B}}}

\newcommand\BurA{Bureaucracy {\textsf {A}}}
\newcommand\BurB{Bureaucracy {\textsf {B}}}

\newcommand\Psyche{\textsc{Psyche}}


